LatentCRF: Continuous CRF for Efficient Latent Diffusion

Latent Diffusion Models (LDMs) produce high-quality, photo-realistic images, however, the latency incurred by multiple costly inference iterations can restrict their applicability. We introduce LatentCRF, a continuous Conditional Random Field (CRF) model, implemented as a neural network layer, that models the spatial and semantic relationships among the latent vectors in the LDM. By replacing some of the computationally-intensive LDM inference iterations with our lightweight LatentCRF, we achieve a superior balance between quality, speed and diversity. We increase inference efficiency by 33% with no loss in image quality or diversity compared to the full LDM. LatentCRF is an easy add-on, which does not require modifying the LDM.

==> tables/ablate_energy.tex <==
\begin{table}[t]
\small
\centering
\caption{\footnotesize
\textbf{CRF Ablation:} 
We report FID scores on the base (FID-B) and large (FID-L) variants of \modelname where sub-components of the CRF are ablated. Removing the pairwise (only unaries) will provide the input directly as the output, so it is omitted. Adding text conditioning (text) to the pairwise energy term and introducing the higher order term consistently improves FID across both \modelname variants.   
}\label{table:ablate_energy}
\vspace{-1.0em}
\def\arraystretch{1.2}  % height
\setlength\tabcolsep{0.7em}  % width
\scalebox{0.85}{
\begin{tabular}{c|c|c|S|S}
\toprule
Pairwise & Text  & Higher Order & \text{FID-B $\downarrow$} & \text{FID-L $\downarrow$} \\ \midrule \rowcolor{Gray}
\cmark  & \cmark & \cmark &  11.58           & 11.27 \\
\cmark  & \cmark & \xmark &  11.62\dec{0.04} & 11.58\dec{0.31} \\ 
\cmark  & \xmark & \xmark &  11.78\dec{0.20} & 11.72\dec{0.45} \\
% \midrule
% LDM-50  & -      & -      &  -        & 12.75 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/ablate_infer.tex <==
\begin{table}[t]
\small
\centering
\caption{
\textbf{Inference Pipeline Ablation:} 
We demonstrate the effects or ablating (one or both of) the `CRF` and the final 2 `Post-CRF` LDM iterations from our inference pipeline. It is evident that both components contribute to image quality. The LDM baseline is reported for comparison purposes.
}\label{table:ablate_infer}
\vspace{-1.0em}
\def\arraystretch{1.2}  % height
\setlength\tabcolsep{0.8em}  % width
\scalebox{0.85}{
\begin{tabular}{l|c|c|c|S}
\toprule
Method  & Pre-CRF & CRF    & Post-CRF & \text{FID $\downarrow$} \\ \midrule \rowcolor{Gray}
Ours    & 31      & \cmark &  2       & 11.58 \\
Ours    & 31      & \cmark &  0       & 11.74\dec{0.16} \\
Ours    & 31      & \xmark &  2       & 19.72\dec{8.14} \\
Ours    & 31      & \xmark &  0       & 21.85\dec{10.27} \\ 
\midrule
LDM  & -      & -      &  -      & 12.75 \\
% LDM-20  & -      & -      &  -      & 12.80 \\ 
\bottomrule
\end{tabular}
}
\end{table}

